DTFormer: A Transformer-Based Method for Discrete-Time Dynamic Graph Representation Learning

Discrete-Time Dynamic Graphs (DTDGs), which are prevalent in real-world implementations and notable for their ease of data acquisition, have garnered considerable attention from both academic researchers and industry practitioners. The representation learning of DTDGs has been extensively applied to model the dynamics of temporally changing entities and their evolving connections. Currently, DTDG representation learning predominantly relies on GNN+RNN architectures, which manifest the inherent limitations of both Graph Neural Networks (GNNs) and Recurrent Neural Networks (RNNs). GNNs suffer from the over-smoothing issue as the models architecture goes deeper, while RNNs struggle to capture long-term dependencies effectively. GNN+RNN architectures also grapple with scaling to large graph sizes and long sequences. Additionally, these methods often compute node representations separately and focus solely on individual node characteristics, thereby overlooking the behavior intersections between the two nodes whose link is being predicted, such as instances where the two nodes appear together in the same context or share common neighbors. This paper introduces a novel representation learning method DTFormer for DTDGs, pivoting from the traditional GNN+RNN framework to a Transformer-based architecture. Our approach exploits the attention mechanism to concurrently process topological information within the graph at each timestamp and temporal dynamics of graphs along the timestamps, circumventing the aforementioned fundamental weakness of both GNNs and RNNs. Moreover, we enhance the model's expressive capability by incorporating the intersection relationships among nodes and integrating a multi-patching module. Extensive experiments conducted on six public dynamic graph benchmark datasets confirm our model's efficacy, achieving the SOTA performance.

==> alg_flow.tex <==
\begin{algorithm}[t]
\caption{\ours~forward computation}
\label{alg:flow}
    \KwIn{DTDG snapshots up to time $t-1$ $\mathcal{G} = \{\mathcal{G}_1, \mathcal{G}_2, \ldots, \mathcal{G}_{t-1} \}$}
    
    \KwOut{Predict the probability of the existence of an edge between nodes $i$ and $j$ at time $t$.}

    % Extract first-hop history neighbor sequences for node $i$ and node $j$.
    $\mathcal{N}_i^{t'}, \mathcal{N}_j^{t'} \leftarrow \mathcal{G}$ 

    % Get basic features from raw data.
    $\mathbf{Node}_{\mathcal{N}_i^{t'}} \leftarrow \mathbf{X}, \mathcal{N}_i^{t'}$;
    $\mathbf{Edge}_{\mathcal{N}_i^{t'}} \leftarrow \mathbf{F}, \mathcal{N}_i^{t'}$; 
    $\mathbf{Node}_{\mathcal{N}_j^{t'}} \leftarrow \mathbf{X}, \mathcal{N}_j^{t'}$;
    $\mathbf{Edge}_{\mathcal{N}_j^{t'}} \leftarrow \mathbf{F}, \mathcal{N}_j^{t'}$.

    
    



    
\end{algorithm}

==> tab_datasets.tex <==
\begin{table*}[t]

\centering

\caption{Summary of datasets metadata.}

\begin{tabular}{cccccc}
\toprule
              & \# Edges & \# Nodes                       & Range                       & \# Snapshots & \# Edge Features \\ \midrule
Bitcoin-OTC   & 35,592   & 5,881                          & Nov 8, 2010 - Jan 24, 2016  & 279   &0       \\
UCI-Message   & 59,835   & 1,899                          & Apr 15, 2004 - Oct 26, 2004 & 29    &0       \\
Reddit-Title  & 571,927  & 54,075                         & Dec 31, 2013 - Apr 30, 2017 & 178   &86       \\
Reddit-Body   & 286,561  & 35,776                         & Dec 31, 2013 - Apr 30, 2017 & 178   &86       \\
Mathoverstack & 506,550  & 24,818 & Sep 29, 2009 - Mar 06, 2016 & 2,350  &0       \\
Email         & 332,334  & 986                            & /                           & 803    &0      \\ \bottomrule
\end{tabular}

\label{tab:datasets}
\end{table*}
